Free Pick functions: representations, asymptotic behavior and matrix monotonicity in several noncommuting variables

We extend the study of the Pick class, the set of complex analytic functions taking the upper half plane into itself, to the noncommutative setting. R. Nevanlinna showed that elements of the Pick class have certain integral representations which reflect their asymptotic behavior at infinity. Loewner connected the Pick class to matrix monotone functions. We generalize the Nevanlinna representation theorems and Loewner's theorem on matrix monotone functions to the free Pick class, the collection of functions that map tuples of matrices with positive imaginary part into the matrices with positive imaginary part which obey the free functional calculus.

==> hardyBackup.tex <==
\subsection{The free coefficient Hardy space}\label{fchardy}
	 Introduced in \cite{har15}, and \cite{har-lit},
	 the classical Hardy space $H^2$ is typically defined as the set of analytic functions
	on the disk so that
		$$\lim_{r\rightarrow 1} \frac{1}{2\pi}\int^{\pi}_{-\pi} |f(re^{i\theta})|\,\dd\theta \leq \infty.$$
	The space $H^2$ is endowed with an inner product given by the formula
		$$\ip{f}{g} = \lim_{r\rightarrow 1} \frac{1}{2\pi}\int^{\pi}_{-\pi} f(re^{i\theta})\overline{g(re^{i\theta})}\,\dd\theta$$
	and is indeed a Hilbert space.
	In an alternative characterization, the functions $z^n$ form an orthonormal basis for $H^2.$ Thus, $H^2$ is
	also the set of functions on the disk such that their coefficients in a power series at the
	origin are sequences in $l^2.$
	
		In the classical Hardy space $H^2,$ there exists a function, the Szeg\"o kernel \cite{sze21b,kra}, $k_\alpha$
	such that if $f \in H^2,$ then
		$$f(\alpha)= \ip{f}{k_\alpha}.$$
	
		We generalize the second interpretation of the Hardy space as the \emph{free coefficient Hardy space}.
	\begin{definition}
		Let $\mathcal{I}$ be the set of monomial indices in the free algebra with $d$ variables.
		The \emph{free coefficient Hardy space} $H^2_d$ is the set of functions $f$ defined on
		matrices of norm less than $\frac{1}{d}$ so that 
			$f(X) = \sum_{I\in \mathcal{I}} a_IX^I$ 
		for some sequence $(a_I)_{I\in \mathcal{I}}\in l^2(\mathcal{I}).$
		The inner product on $H^2_d$ is inherited from the underlying coefficient space $l^2(\mathcal{I}).$
	\end{definition}
	
		Importantly, this space has a Szeg\"o kernel itself.
	\begin{definition}\label{szego}
		Let $\mathcal{I}$ be the set of monomial indices in the free algebra with $d$ variables.
		Let $X \in \M^n.$
		Define the monomial basis vector $m_X = (X^I)_{I\in \mathcal{I}}.$
		The Szeg\"o kernel is given by $k^{ij}_X = (\overline{(m^X_{I})_{ij}})_{I\in \mathcal{I}}.$ That is, it is the sequence
		$(i,j)$-th entries of each monomial $I$ evaluated at $X.$
	\end{definition}
		Note that by a straightforward calculation,
			$$f(X)_{ij} = \ip{f}{k^{ij}_X}.$$
		Thus, the behavior of $f$ at $X$ is determined by the projection of $f$
		onto the space spanned by $k^{ij}_X.$
	\begin{definition}\label{szegospace}
		Define 
			$$V_X = \operatorname{span}_{ij}\{k^{ij}_X\} \subset H^2_d.$$
		Furthermore, define $P_X: H^2_d \rightarrow V_X$ to be the projection onto $V_X.$
%		\red I don't see any motivation for giving these a name at this juncture, if other people think they're useful, they'll give them a name, but i dont thin it adds anything. \black 		
%		\blue I want to be more precise about this. For functions in the space $H^2_d$,  at a point $X$ define by $P_X$ the local projection onto $V_X$? \black  
	\end{definition}
		Thus, given some pair $(X, Y)$ such that there is a free polynomial with $p(X) = Y$,
		we can correspond to $p$ a unique $f$ of minimum norm in $H^2_d$ such that $f(X) = Y$ by assigning
		$f = P_X p.$
	
		The following is essentially the statement that the values of a function determine the function.
	\begin{proposition}\label{denseSpan}
		$$\overline{\bigcup_{\|X\|\leq \frac{1}{d}} V_X} = H^2_d.$$ 
	\end{proposition}
	\begin{proof}
		Suppose $\overline{\bigcup_{\|X\|\leq \frac{1}{d}} V_X} \neq H^2_d.$ Then there exists a nonzero function
		$f \in\overline{\bigcup_{\|X\|\leq \frac{1}{d}} V_X}^\perp.$
		So, $0 = \ip{f}{k^{ij}_X}$ for all $i, j$ and $X$ which implies that $f$ is zero. Contradiction.
	\end{proof}
		In general we will often forget coordinate systems, so we use an alternative characterization of $V_X.$
	\begin{proposition}\label{altszegspace}
		The space $V_X$ is the unique vector space such that
		$$\tensor{V_X}{\mathbb{C}^n} = \mathrm{span}\{\tensor{I}{U} m_Xc| c \in \mathbb{C}^n, U \in U_n\}.$$
	\end{proposition}
	To prove this we need a decomposition theorem, a \emph{detensoring lemma} that will allow us to show that spaces like the one
	in the above lemma are well defined.
	\begin{lemma}[Detensoring lemma]\label{stsc}
		Let $V$ be a subspace of $\tensor{\hilbert}{\mathbb{C}^n}$ such that if $U \in U_n$ then
		$$\tensor{I}{U} V = V.$$ Then there exists $V'$, a subspace of $\hilbert$, so that $V = \tensor{V'}{\mathbb{C}^n}.$
	\end{lemma}
	\begin{proof}
		Let $e_1, \ldots, e_n$ be an orthonormal basis for $\mathbb{C}^n.$
		
		Let $V'$ be the subspace $\{v | \tensor{v}{e_1} \in V\}.$
		
		We first show $V \subseteq V'\otimes \mathbb{C}^n.$
		Let $v \in V.$
		Then $$v = \sum_i \tensor{v_i}{e_i}.$$
		Let $U_i$ be the unitary that fixes $e_i$ and sends $e_j$ to $-e_j$ if $i \neq j.$
		So, $$\tensor{I}{U_i}v  = \sum_i (-1)^{\chi(i\neq j)} \tensor{v_i}{e_i} \in V$$ by assumption. Therefore
		$\frac{1}{2}\left(\tensor{I}{U_i}v + v\right) = \tensor{v_i}{e_i} \in V.$ Let $W_i$ be a unitary taking $e_i$ to $e_1.$
		So $$\tensor{I}{W_i}\tensor{v_i}{e_i} = \tensor{v_i}{e_1}.$$
		Thus, each $v_i \in V'$ and so $v \in \tensor{V'}{\mathbb{C}^n}$.
		
		We now show $V \supseteq \tensor{V'}{\mathbb{C}^n}.$
		Suppose $v \in \tensor{V'}{ \mathbb{C}^n},$
		so that, $$v = \sum_i \tensor{v_i}{e_i}$$ where each $v_i \in V'.$ Let $W_i$ be a unitary taking $e_1$ to $e_i.$
		Thus, $$v = \sum_i \tensor{I}{W_i} \tensor{v_i}{e_1} \in V$$ since each $\tensor{I}{W_i}
		\tensor{v_i}{e_1} \in V$ by definition.
	\end{proof}
	
	We now prove Proposition \ref{altszegspace}.
	\begin{proof}[Proof of Proposition \ref{altszegspace}]
		By the detensoring lemma, there is a unique vector space $V$ such that
			$$\tensor{V}{\mathbb{C}^n} = \mathrm{span}\{\tensor{I}{U} m_Xc| c \in \mathbb{C}^n, U \in U_n\}.$$
		
		Let $U_1$ be the unitary sending $e_i$ to $-e_i$. 
		Note, 
		$$\tensor{k_X^{ij}}{e_i} = \frac{1}{2}\left[\tensor{I}{I}m_Xe_j - \tensor{I}{U_1}m_Xe_j\right].$$  Thus, $V$ contains $V_X$ as the $k_X^{ij}$ form a basis for $V_X.$
		
		Let $E_{ij}$ designate the matrix in $\M_n$ with $1$ in the $ij$th position and $0$ elsewhere. Note, $m_X = \sum \tensor{k_X^{ij}}{E_{ij}}.$
		So, since unitaries in $\M_n$ span $\M_n$ itself, it can be derived that
			$$\mathrm{span}\{\tensor{I}{U} m_X W| U, W \in U_n\}= \mathrm{span}\{ \tensor{k_X^{ij}}{A} | A \in \M_n \}.$$
		Now, if $f \in V,$ there is some $l\in \mathbb{C}^n$ such that
			$$\tensor{f}{l} = \sum_{ij} \tensor{k_X^{ij}}{A}c_{ij}.$$
		Note that $Ac_{ij} = l,$ since $k_X^{ij}.$ So
			$\tensor{f}{l} = \sum_{ij} \tensor{k_X^{ij}}{l}.$
		So $\tensor{V}{\mathbb{C}^n} \subseteq \tensor{V_X}{\mathbb{C}^n}$ and thus $V_X$ contains $V$.
	\end{proof}
	
	\subsubsection{Example: the free coefficient Hardy space in one variable}
		We will now compute some of the previous definitions
		in the free coefficient Hardy space in one variable, $H^2_1.$ 
		
		Under the characterization of the classical Hardy space in terms of its power series,
		the free coefficient Hardy space $H^2_1$ in one variable is essentially the same object as the
		classical Hardy space, where one is allowed to evaluate functions in $H^2$ on contractions.
		
		For some nonzero $\lambda$ sufficiently close to zero, the matrix
			$$X = \left(\begin{matrix}
			\lambda & \lambda \\
			0 & \lambda 
			\end{matrix}\right)$$
		has norm less than $1,$ and so we can compute the associated objects to $X$ given in Definitions
		\ref{szego} and \ref{szegospace}. 
		To compute the Szeg\"o kernel defined in Definition \ref{szego}, we
		note that
			$$X^n = \left(\begin{matrix}
			\lambda^n & n\lambda^n \\
			0 & \lambda^n 
			\end{matrix}\right)$$
		and thus as vectors of coefficients,
			$$k^{11}_X=k^{22}_X =
			\left(\begin{matrix}
			1 \\
			\overline{\lambda} \\
			\overline{\lambda^2} \\
			\vdots
			\end{matrix}\right),
			k^{12}_X =
			\left(\begin{matrix}
			0 \\
			\overline{\lambda} \\
			\overline{2\lambda^2} \\
			\vdots
			\end{matrix}\right), k_X^{21} = 0.
			$$
		
		In the work of Helton, Klep and McCullough \cite{helkm11} and in Kaliuzhnyi-Verbovetskyi and Vinnikov \cite{vvw12}, one finds a formula for
		computing the derivative of a free function using the value of the freee function itself at some specially
		constructed point. In our case, we obtain the following
			$$f\left(\begin{matrix}
			\lambda & \lambda \\
			0 & \lambda
			\end{matrix}\right)
			=
			\left(\begin{matrix}
			f(\lambda) & \lambda f'(\lambda) \\
			0 & f(\lambda)
			\end{matrix}\right).$$
		If $f(z) = \sum a_iz^i,$ then computing
			$$ \begin{matrix}
			f\left(\begin{matrix}
			\lambda & \lambda \\
			0 & \lambda
			\end{matrix}\right)& = &
			\left(\begin{matrix}
			\ip{f}{k^{11}_X} & \ip{f}{k^{12}_X} \\
			\ip{f}{k^{11}_X} & \ip{f}{k^{22}_X}
			\end{matrix}\right) \\
			& = &
			\left(\begin{matrix}
			\sum a_i\lambda^i & \sum ia_i\lambda^i \\
			0 & \sum a_i\lambda^i
			\end{matrix}\right) \\
			& = & 
			\left(\begin{matrix}
			f(\lambda) & \lambda f'(\lambda) \\
			0 & f(\lambda)
			\end{matrix}\right)
			\end{matrix}
			$$
		agrees with the previous formula. Thus, the value at $X$ determines the value of $f(\lambda)$ and $f'(\lambda)$ and vice versa.
		These two degrees of freedom are again reflected in the fact that $V_X$ is two dimensional.
		
		Explicitly computing $k^{11}_X$ and $k^{12}_X$ as functions gives
			$$k^{11}_X(z) = \frac{1}{1-\overline{\lambda} z},
			k^{11}_X(z) = \frac{\overline{\lambda}^2}{(1-\overline{\lambda} z)^2}.$$
			
		Consider the interpolation problem of finding an $f \in H^2_1,$ $f(\lambda) = a$ and $f'(\lambda) = b.$
		We find that the minimum norm function satisfying this interpolation problem is of the form
			$$f(z) = \mu_1\frac{1}{1-\overline{\lambda} z} + \mu_2\frac{\overline{\lambda}^2}{(1-\overline{\lambda} z)^2}.$$
		
		
		To find $\mu_1$ and $\mu_2$ in the above problem explicity, we compute the projection $P_X.$
		This can be accomplished via a formula given in Horn and Johnson \cite{horjoh85}.
		Let
			$$K = (\begin{matrix}k^{11}_X & k^{12}_X \end{matrix})$$
		then the desired projection is given by a formula
			$$P_X = K(K^*K)^{-1}K^*.$$
		Thus if $f$ is the desired function
			$P_Xf =f$ and so
		$$
			\left(\begin{matrix} \mu_1 \\
			\mu_2 \\
			\end{matrix}\right)
			=
			(K^*K)^{-1}K^*f.$$
		The object $K^*K$ is the Grammian of the vectors $k^{11}_X, k^{12}_X$ and is given by
			$$K^*K = \left(\begin{matrix}\ip{k^{11}_X}{k^{11}_X} & \ip{k^{11}_X}{k^{12}_X} \\
			\ip{k^{12}_X}{k^{11}_X} & \ip{k^{12}_X}{k^{12}_X} \\
			\end{matrix}\right) = 
			\left(\begin{matrix}\frac{1}{1-|\lambda|^2} & \frac{\lambda^2}{(1-|\lambda|^2)^2}  \\
			\frac{\overline{\lambda}^2}{(1-|\lambda|^2)^2} & \frac{1+|\lambda|^2}{(1-|\lambda|^2)^3} \\
			\end{matrix}\right).$$
		So,
			$$(K^*K)^{-1} = \frac{1}{1 +|\lambda|^2 - |\lambda|^4}
			\left(\begin{matrix} (1+|\lambda|^2)(1-|\lambda|^2) & -\lambda^2(1-|\lambda|^2)^2  \\
			-\overline{\lambda}^2(1-|\lambda|^2)^2 &  (1-|\lambda|^2)^3 \\
			\end{matrix}\right).$$
		Note that $K^*f = \left(\begin{matrix}f(\lambda) \\ \lambda f'(\lambda)\end{matrix}\right) =
		\left(\begin{matrix}a \\ \lambda b\end{matrix}\right),$ so $\mu_1$ and $\mu_2$ are given by the formula
			$$
			\left(\begin{matrix} \mu_1 \\
			\mu_2 \\
			\end{matrix}\right)
			=
			\frac{1}{1 +|\lambda|^2 - |\lambda|^4}
			\left(\begin{matrix} a(1+|\lambda|^2)(1-|\lambda|^2) + -b\lambda^3(1-|\lambda|^2)^2  \\
			-a\overline{\lambda}^2(1-|\lambda|^2)^2 +  b\lambda(1-|\lambda|^2)^3 \\
			\end{matrix}\right).$$
		
	\subsubsection{The coefficient Hardy space of a general free vector-valued function}
		The free coefficient Hardy space is useful for interpolation problems to obtain existence
		and uniqueness results. If we relax the choice of basis of functions, we still obtain
		uniqueness results. For our constructions, this is often enough.
			
		\begin{definition}
		Let $\ph$ be a free function on a domain $D \subset \M^d$ and taking values in $\tensor{\hilbert}{\M}$.
		The \emph{free coefficient Hardy space for $\ph$}, $H^2_\ph$, is the set of functions $f$ defined on
		$D$ so that 
			$$f(X) = \tensor{u^*}{I}\ph(X)$$
		for some vector $u \in \hilbert.$ 
%		\red Seems like the paragraph above does this to me. \black 		
%		\blue You should clarify with a sentence why this expression is equivalent to the power series setup. It's %not immediately obvious what the motivation is for this definition and it's important enough to waste the time with %a motivator. \black
		Decompose $$\hilbert = \hilbert_1 \oplus \{u\in \hilbert|\forall X\in D, \tensor{u^*}{I}\ph(X) = 0\}$$
		The inner product on $H^2_\ph$ is inherited from the underlying inner product on $\hilbert_1.$
		\end{definition}
	
		We define the vector spaces from Definition \ref{szegospace} in the second abstract characterization which is easier to
		state in this context. However, a choice of basis will yield Szeg\"o kernels as in the original definition.
		\begin{definition} \label{localvec}
		Let $\ph$ be a free function on a domain $D \subset \M^d$ and taking values in $\tensor{\hilbert}{\M}$, and let $X \in \M^d_n.$
		The space $V^\ph_X \subset H^2_{\ph}$ is the unique vector space such that
		$$\tensor{V^\ph_X}{\mathbb{C}^n} = \mathrm{span}\{\tensor{I}{U} \ph(X)c| c \in \mathbb{C}^n, U \in U_n\}.$$
		
		Define the projection $P^\ph_X: H^2_\ph \rightarrow V^\ph_X$ to be the projection onto $V^\ph_X.$
		\end{definition}
		
		We note again that for $f,g \in H^2_\ph,$ $f(X) = g(X)$ if and only if $P^\ph_Xf=P^\ph_Xg.$
	Furthermore, the spaces $V^{\ph}_X$ exhaust $H^2_\ph.$
	\begin{proposition}\label{denseSpanGen}
		$$\overline{\bigcup_{X\in D} V^{\ph}_X} = H^2_\ph.$$ 
	\end{proposition}
	\begin{proof}
		Suppose $f \in (\bigcup_{X\in D} V^{\ph}_X)^{\perp}.$
		So, for every $X,$ $P_X f = 0 = P_X 0.$ Thus, $f(X) \equiv 0.$
	\end{proof}
	
	
	


==> herglotzBackup.tex <==
\subsection{Models and representations of free Herglotz functions}


Connections between the various special classes of functions that we consider are given by the \emph{Cayley transform}. The particular Cayley transform given by
\[
	\la = \frac{z - 1}{z + 1}, \,\, z = \frac{1 + \la}{1 - \la}
\]
is a conformal mapping between the right half-plane and the disk. We will apply this transform to the free Schur model in \eqref{ncschur} to develop a model for free Herglotz functions.\foot{Herglotz functions were characterized by C. Carath\'eodory in \cite{car07} and given an integral representation by Gustav Herglotz in \cite{herg11}. J. Agler generalized this representation for functions in the so-called $d$-variable strong Herglotz class, a conformal equivalent of the Schur-Agler class, in \cite{ag90}.} Recall that a Herglotz function is a holomorphic function $h$ on $\D$ with $\RE h \geq 0$ (It is often convenient to normalize Herglotz functions so that $h(0) = 1$). 
 
To define free Herglotz functions, we need an analogue of the right halfplane. Denote by $\Psi \subset \M$ the right matrix polyhalfplane
\[
	\Psi = \{X \in \M | \RE X > 0\}.
\]

We take our definition of a free Herglotz function $h$ to be a free holomorphic function from the matrix ball $\B^d \to \Psi$. 

We require the following lemma in our proof of the existence of models of free Herglotz functions. 
\begin{lemma} \label{herglotzunitary}
	Let $\hilbert_1$ and $\hilbert_2$ be Hilbert spaces, let $W$ be a bounded operator on $\hilbert_1 \oplus \hilbert_2$ with block form
	\[
		W = \bbm A & B \\ C & D \ebm,
	\]
	assume that $1 \notin \sigma(A)$, and let $U = D - C(1+A)\inv B$. If $W$ is an isometry then so is $U$, and if $W$ is unitary then so is $U$. 
\end{lemma}

The representation of a classical Herglotz function $h$ with $h(0) = 1$ is given by a probability measure $\mu$ on the unit circle so that
	$$h(z) = \int_0^{2\pi} \frac{1 + e^{-i\theta}}{1 - e^{-i\theta}} \,\dd\mu(\theta).$$
The following theorem gives an analogous formula in the free case.

\begin{theorem}
	Let $h$ be a free holomorphic function with $h(0) = 1$. $h:\B^d \to \Psi$ if and only if there exist a Hilbert space $\hilbert_d = \oplus_{i=1}^d \hilbert$, a unitary operator $U$ on $\hilbert_d$ and an isometry $V: \C \to \hilbert_d$ so that 
		\beq \label{herglotz}
		h(X) = \tensor{V\ad}{I} \left( I + \tensor{U}{I}\delta(X)\right)\left( I - \tensor{U}{I}\delta(X)\right)\inv \tensor{V}{I}, 
		\eeq
	where 
		$$\delta(X): \M^d \to \tensor{\hilbert_d}{\M} = \bigoplus_{i=1}^d \tensor{I}{X^i}$$.
\end{theorem}

\begin{proof}
	Key ideas in our proof follow Agler \cite{ag90}. 

	$\Rightarrow:$ Suppose that $h$ is a free Herglotz function. Then under the Cayley transform, define the corresponding free Schur function $\phi:\B^d \to \B$ by
	\[
		\phi(X) = (h(X) - I)(h(X) + I)\inv.
	\]
	By Theorem \ref{ncschur}, for any $X, Y \in \B^d_n$,
	\[
		1 - \phi(Y)\ad\phi(X) = \sum_i u_i(Y)\ad\tensor{I}{I - Y_i\ad X_i}u_i(X),
	\] 
	which after substitution becomes
	\[
		1 - [(h(Y) - I)(h(Y) + I)\inv ]\ad(h(X) - I)(h(X) + I)\inv = \sum_i u_i(Y)\ad\tensor{I}{I - Y_i\ad X_i}u_i(X).
	\]
	Multiplying on the left and right by $(h(Y) + I)\ad$ and $(h(X) + I)$ respectively, we get
	\begin{align*}
		(h(Y) + I)\ad &(h(X) + I) - (h(Y) - I)\ad (h(X) - I) \\ &= \sum_i (h(Y) + I)\ad u_i(Y)\ad \tensor{I}{I - Y_i\ad X_i} u_i(X) (h(X) + I) \\
		&= \sum_i \left[u_i(Y)(h(Y) - I)\right]\ad \tensor{I}{I - Y\ad_i X_i} \left[u_i(X) (h(X) + I)\right].
	\end{align*}
Let $v_i(X) = u_i(X)(h(X) + I)$. Upon substitution and rearrangement, the above equation becomes
\begin{align*}
(h(Y) + I)\ad(h(X) + I) + &\sum_i v_i(Y)\ad \tensor{I}{Y\ad_i X_i} v_i (X) \\&= (h(Y) - I)\ad(h(X) -I) + \sum_i v_i(Y)\ad v_i(X).
\end{align*}
This equation can be rewritten as
\begin{align}
(h(Y) + I)\ad (h(X) + I) &+ \sum_i \left(\tensor{I}{Y_i} v_i(Y)\right)\ad \left(\tensor{I}{X_i} v_i(X) \right) \notag \\ &= (h(Y) - I)\ad(h(X) - I) + \sum_i v_i(Y)\ad v_i(X) \label{sorted}.
\end{align}
Let
\[
v(X) = \bbm v_1(X) \\ \vdots \\ v_d(X) \ebm,
\]
and let $\delta(X)$ be the operator in $\tensor{\B(\hilbert_d)}{\M}$ given by
\[
\delta(X) = \bigoplus_{i=1}^d \tensor{I}{X_i}.
\] 
Then we can rewrite \eqref{sorted} as
\beq \label{gramian}
\vectwo{h(Y) + I}{\delta(Y)v(Y)}\ad\vectwo{h(X) + I}{\delta(X)v(X)} = \vectwo{h(Y) - I}{v(Y)}\ad\vectwo{h(X) - I}{v(X)}  \, \begin{array}{c} \M \\ \tensor{\hilbert_d}{\M} \end{array}.
\eeq
Noting that $\M = \tensor{\C}{ \M}$, and given that
\[
\vectwo{\tensor{\C}{\M}}{\tensor{\hilbert_d}{\M}} \cong \tensor{\C \oplus \hilbert_d}{\M},
\]
we view \eqref{gramian} as a relation between vectors in $\tensor{\C \oplus \hilbert_d}{\M}$. Let 
	$$\phi(X) = \vectwo{h(X) + I}{\delta{X}v(X)}, \text{ and } \theta(X) = \vectwo{h(X) - I}{v(X)}.$$
Then by Theorem \ref{lurk}, there exists an isometry $U$ such that
	$$\tensor{U}{I}\phi(X) = \theta(X)$$.

 there exists a unitary operator $L$ defined by
\[
L = \begin{bmatrix} A & B \\ C & D \end{bmatrix} \begin{array}{c} \C \\ \hilbert_d \end{array}
\]
so that 
\[
\bbm \tensor{A}{I} & \tensor{B}{I} \\ \tensor{C}{I} & \tensor{D}{I} \ebm \vectwo{h(X) + I}{\delta(X)v(X)} = \vectwo{h(X) - I}{v(X)}.
\]
Multiplying through gives the relations
\begin{align*}
&\tensor{A}{I} (h(X) + I) + \tensor{B}{I} \delta(X)v(X) =  (h(X) - I), \\
&\tensor{C}{I} (h(X) + I) + \tensor{D}{I} \delta(X)v(X) =  v(X).
\end{align*}

Arranging this system to facilitate elimination of $h$, we get
\begin{align*}
\tensor{I + A}{I} &h(X) + \tensor{B}{I}\delta(X)v(X) = \tensor{I - A}{I} \\
\tensor{C}{I}&h(X) + \left(\tensor{D}{I}\delta(X) - I\right)v(X) = \tensor{-C}{I}.
\end{align*}
Multiplying through the first equation by $\tensor{(I + A)\inv}{I}$ and then $\tensor{C}{I}$ gives the system
\begin{align*}
\tensor{C}{I} &h(X) + \tensor{C(I + A)\inv B}{I}\delta(X)v(X) = \tensor{C(I+A)\inv (I - A)}{I} \\
\tensor{C}{I}&h(X) + \left(\tensor{D}{I}\delta(X) - I\right)v(X) = \tensor{-C}{I}.
\end{align*}
Subtracting the equations to eliminate $h(X)$,
\[
\left[I - \left(\tensor{D}{I} - \tensor{C(I+A)\inv B}{I}\right)\delta(X)\right]v(X) = \tensor{C(I + A)\inv (I - A) + I}{I},
\]
which upon application of Lemma \ref{herglotzunitary} and after simplification becomes
\[
\left(I - \tensor{U}{I}\delta(X)\right)v(X) = \tensor{2C(I+A)\inv}{I}.
\]
Let $V = C(I+A)\inv \in \B(\C, \hilbert_d)$. Then we get the following expression for $v(X)$:
\beq \label{sub1}
v(X) = \left(I - \tensor{U}{I}\delta(X)\right)\inv \tensor{2V}{I}.
\eeq
Another useful form of this equation is
\beq \label{sub2}
v(X) = \tensor{U}{I}\delta(X)v(X) + \tensor{2V}{I}.
\eeq



Expression \eqref{sorted} can be rewritten as 
\beq \label{simplesorted}
2(h(Y)\ad + h(X)) =  v(Y)\ad v(X) - (\delta(Y)v(Y))\ad\delta(X)v(X).
\eeq
So, using \eqref{sub2}, we have 
\beq \label{almostrep}
2(h(Y) + h(X)) = \left(\tensor{U}{I}\delta(Y)v(Y)\right)\ad\tensor{2V}{I} + \tensor{2V\ad U}{I}\delta(X)v(X) + \tensor{2V\ad}{I}\tensor{2V}{I}.
\eeq

As $h(0) = I$, upon setting $X,Y = 0$, the equation above becomes
\[
4 = \tensor{2V\ad}{I} \tensor{2V}{I},
\]
and so $V\ad V = I$ which shows that $V$ is an isometry.
Now set $Y = 0$ in \eqref{almostrep} and divide by $2$. Then
\[
h(X) = \tensor{V\ad}{I}\tensor{U}{I}\delta(X)v(X) + I.
\]
By \eqref{sub1},
\begin{align*}
h(X) &= \tensor{V\ad}{I}\tensor{U}{I}\delta(X)\left(I - \tensor{U}{I}\delta(X)\right)\inv \tensor{2V}{I} + I \\
&= \tensor{V\ad}{I}\left[2\tensor{U}{I}\delta(X)\left(I - \tensor{U}{I}\delta(X)\right)\inv + I\right]\tensor{V}{I} \\
&= \tensor{V\ad}{I}\left[\left(I + \tensor{U}{I}\delta(X)\right)\left(I - \tensor{U}{I}\delta(X)\right)\inv\right]\tensor{V}{I}.
\end{align*}
Thus we have shown that a free Herglotz function has a model. We note that the isometry $V$ is a map from $\C \to \hilbert_d$, and  to emphasize that $V$ is rank one, we will use the vector notation $V = v$ and $V\ad = v^*$ in the following sections.

$\Leftarrow:$ Let $h$ have a model as in \eqref{herglotz}. Let $X \in \B^d$. Then $\delta(X)$ is a contraction on $\hilbert_d$, as is $\tensor{U}{I}\delta(X)$. The expression 
	$$\left(I + \tensor{U}{I}\delta(X)\right)\left(I - \tensor{U}{I}\delta(X)\right)\inv$$
is the Cayley transform of a contraction, and thus has positive real part, i.e. is in $\Psi$ for all $X$. This condition is preserved by isometric conjugation. Thus if $X \in \B^d$, then $h(X) \in \Psi$, and so $h$ is a free Herglotz function.
\end{proof}

\begin{corollary} \label{altherg}
If $h$ is a free Herglotz function on $\B^d$, then there exists a Hilbert space $\hilbert_d = \oplus_i \hilbert_i$, a real constant $a$, a unitary operator $L \in \B(\hilbert_d)$, and a vector $v \in \hilbert_d$ such that for all $X \in \B^d$, 
\beq 
h(X) = -i\tensor{a}{I} + \tensor{v\ad}{I}\left(\tensor{L}{I} - \delta(X)\right)\inv\left(\tensor{L}{I} + \delta(X)\right)\tensor{v}{I},
\eeq
where $\delta(X) = \bigoplus_{i=1}^d \tensor{I}{X_i}$.

Conversely, any $h$ defined by an equation of the form \eqref{altherg} is a free Herglotz function.
\end{corollary}


==> introductionBackup.tex <==
\section{Introduction}
Let $\M^d$ denote the \emph{$d$-dimensional matrix universe}, defined by
\[
\M^d = \bigcup_{n=1}^{\infty} \M_n^d(\C).
\]
\begin{definition}
A set $D \subset \M^d$ is called a \emph{free set} if satisfies the following conditions.
\begin{description}
\item[$D$ is closed with respect to direct sums] 
\hfill
 
$X = (X_1, \ldots, X_d) \in D$ and $Y = (Y_1, \ldots, Y_d) \in D$ if and only if
$
\bpm X & \phantom 0 \\ \phantom 0 & Y \epm = \left(\bpm X_1 & \phantom 0 \\ \phantom 0 & Y_1 \epm, \ldots, \bpm X_d & \phantom 0 \\ \phantom 0 & Y_d \epm\right) \in D.
$
\item[$D$ is closed with respect to unitary similarity]
\hfill

If $X \in D\bigcap \M_n^d, U \in U_n$, then
\[
U\ad X U = (U\ad X_1 U, \ldots, U\ad X_d U) \in D.
\]
\end{description}
Here, $U_n$ denotes the unitary matrices of size $n$.
\end{definition}
\begin{definition}
Let $D$ be a free set.
Let $f: D \to \M^1$ be a function. We say that $f$ is a \emph{free function} if it satisfies the following conditions.
\begin{description}
\item[$f$ is graded] If $X \in D \bigcap \M_n^d$, then $f(X) \in \M_n^1$.
\item[$f$ respects direct sums] If $X, Y \in D$ then
\[ 
f \bpm X & \phantom{0} \\ \phantom 0 & Y \epm = \bpm f(X) & \phantom 0 \\ \phantom 0 & f(Y) \epm.
\]
\item[$f$ respects similarity] 
\hfill

If $S \in GL_n,$ and $X \in D$ such that $S^{-1}XS \in D$, 
\[
f(S\inv X S) = S\inv f(X) S.
\]
\end{description}
Here, $GL_n$ denotes the invertible matricies of size $n$.
\end{definition}


We specify an ordering on matrices where
$A> B$ means $A-B$ is strictly positive definite, and $A \geq B$ means $A-B$ is positive semidefinite.


We consider the \emph{free Pick class} $\mathcal{P}_d,$ functions defined on the domain
\[
\Pi^d := \{X \in \M^d | \IM X_i > 0, i = 1\ldots, d\}
\]
with range in $\cc{\Pi^1}$.
These functions directly generalize multivariable Pick functions, maps from the polyupperhalfplane $\Pi_1^d$ to the upper halfplane $\cc{\Pi_1^1}$.

The structure of classical Pick functions in one variable is very well understood.
%\red reference Ahlfors here? came up in schwarz discussion \black.
Mathematicians of the early 20th century developed the theory within the context of modern analysis \cite{ju20, car29, nev22}.
Pick functions also have deep connections to science and engineering.\cite{alcober,osaka,wigner,Jorswieck2007f, Boche2004e, ahls}

In 1922, Rolf Nevanlinna showed the following theorems \cite{nev22}.

\begin{theorem}[R. Nevanlinna \cite{nev22}]
Let $h: \Pi_1^1 \to \C$. Then $h$ is a Pick function if and only if there exist $a \in \R, b \geq 0$ and a finite positive Borel measure $\mu$ on $\R$ such that 
\[
h(z) = a + bz + \int\!\frac{1 + tz}{t - z}\, \dd\mu(t)
\]
for all $z \in \Pi_1^1$. Moreover, for any Pick function $h$, the numbers $a \in \R, b \geq 0$ and the measure $\mu \geq 0$ are uniquely determined.
\end{theorem}

Furthermore, Nevanlinna showed that a simpler representation, characterizing the Cauchy transforms of positive measures $\mu$ on $\R$, exists as long as $h$ satisfies a mild growth condition as $z \to \infty$. The growth condition is essentially equivalent to saying that the value of $h$ at $z = \infty$ is $0$ and that the first residue exists at $\infty$.
\begin{theorem}[R. Nevalinna \cite{nev22}]
Let $h: \Pi_1^1 \to \C$. There exists a finite positive measure $\mu$ on $\R$ such that 
\[
h(z) = \int\!\frac{\dd\mu(t)}{t-z}d\mu(t)
\]
if and only if $h$ is in the Pick class and
\[
\liminf_{s\to\infty} s\abs{h(is)} < \infty.
\]
\end{theorem}
These two representations, which we refer to as Nevanlinna representations, were recently generalized to several variables in the work of Agler, {\mc}Carthy, and Young \cite{amyloew}, and later in Agler, Tully-Doyle, and Young for multivariable Pick functions that are also in the so-called L\"owner class \cite{aty12,aty13}. 

The $d$-variable L\"owner class $\mathcal L_d$ is the set of analytic functions that lift via the functional calculus to act on $d$-tuples of commuting operators with the property that they possess analytic extensions that take $\Pi^d \to \Pi$.  In the case of one-variable Pick functions, the L\"owner class is the the entire Pick class by von Neumann's inequality \cite{vonN51, szn-foi}. For two variables, the classes coincide by And\^o's Theorem \cite{and63}. In three or more variables, the L\"owner class is a proper subset of the Pick class \cite{par70} \cite{var74}. The L\"owner class is conformally equivalent to the well-studied Schur-Agler class under a double Cayley transform.

The final form of the Nevanlinna representations discussed in \cite{aty13} partitions the L\"owner class into four types. Note that these not only give representations of Pick functions, but also give formulas for constructing new Pick functions.
\begin{definition}
A \emph{positive decomposition} is a collection of positive operators $Y_1, \ldots, Y_d$ on $\hilbert$ so that $\sum_i Y_i = I_\hilbert$, and the operator $z_Y: \C^d \to \hilbert$ is given by 
\[
z_Y = \sum_{i=1}^d z_i Y_i.
\] An \emph{orthogonal decomposition} is a positive decomposition where each $Y_i$ is a projection.
\end{definition}

\begin{theorem}[Agler, Tully-Doyle, Young \cite{aty13}]\label{oldnevreps}
The following are the four types of representations for functions in $\mathcal L_d$. 
\begin{description}
\item[Type 4]  Let $h$ be a function defined on $\Pi_1^d$. Then $h \in \mathcal L_d$ if and only if there exist an orthogonally decomposed
Hilbert space $\hilbert$ and a vector $v \in \hilbert$ such that 
\[
h(z) = \ip{M(z)v}{v},
\]
where $M(z)$ is the matricial resolvent as defined in Proposition 3.1 in \cite{aty13}.
\item[Type 3] Let $h$ be defined on $\Pi_1^d$. Then there exist $a \in \R$, a Hilbert space $\hilbert$, a self-adjoint operator $A$ on $\hilbert$, a vector $v \in \hilbert$, and a positive decomposition
%
%
 $Y$ of $\hilbert$ so that
\[
h(z) = a + \ip{(1-iA)(A- z_Y)\inv(1 + z_Y A)(1 - iA)\inv v}{v}
\]
if and only if $h \in \mathcal L_d$ and
\[
\liminf_{s\to\infty} \frac{1}{s} \IM h(is, \ldots, is) = 0.
\]
\item[Type 2]  Let $h$ be defined on $\Pi_1^d$. Then there exist $a \in \R$, a Hilbert space $\hilbert$, a self-adjoint operator $A$ on $\hilbert$, a vector $v \in \hilbert$, and a positive decomposition $Y$ of $\hilbert$ so that
\[
h(z) = a + \ip{(A - z_Y)\inv v}{v}
\]
if and only if $h \in \mathcal L_d$ and
\[
\liminf_{s \to \infty} s \IM h(is, \ldots, is) < \infty.
\]
\item[Type 1]  Let $h$ be defined on $\Pi^d_1$. Then there exist a Hilbert space $\hilbert$, a self-adjoint operator $A$ on $\hilbert$, a vector $v \in \hilbert$, and a positive decomposition $Y$ of $\hilbert$ so that 
\[
h(z) = \ip{(A - z_Y)\inv v}{v}
\]
if and only if $h \in \mathcal L_d$ and
\[
\liminf_{s \to \infty} s\abs{h(is, \ldots, is)} < \infty.
\]
\end{description}
\end{theorem}

We show that free Pick functions also satisfy the above theorem. Our Theorem \ref{newnevrep} is a precise analogue of Theorem \ref{oldnevreps} in the noncommutative setting. This is an example of \emph{noncommutative lifting principle}, a guiding principle that states that if a theorem holds by virtue of operator theoretic methods following  Agler's seminal paper of 1990, \emph{On the representation of certain holomorphic functions defined on a polydisc}, then it will hold for free functions. Our proofs of these theorems illustrate the theme of lifting functions from varieties to whole domains which began with Cartan's theorems A and B \cite{car51} and continued in \cite{agmc_vn} with bounds and later more precisely by \cite{agmc_dv, jkmc}, etc.

The notion of a Hilbert space model of a function has been the primary tool used to study the L\"owner class and the conformally equivalent Schur-Agler class\cite{ag90, amyloew}. These give a technical description of a function which interfaces well with operator theory.
%Many can be found in Agler \cite{ag90}.
%In the context of this discussion, a model is a map from the domain of a function into some Hilbert space such that a certain identity holds.
%\begin{theorem}[Agler \cite{ag90}, Agler, {\mc}Carthy, Young\cite{amyloew}]
%\hfill
%\begin{enumerate}
%\item Let $\ph$ be a function defined on $\D^d$. Then there exist an orthogonally decomposed Hilbert space $\hilbert = \hilbert_1, \ldots, \hilbert_d$ and an analytic map $u: \D^d \to \hilbert$ such that
%\[
%1 - \cc{\ph(\mu)}\ph(\la) = \sum_{i=1}^d (1 - \cc\mu_i\la_i)\ip{u_i(\la)}{u_i(\mu)},
%\]
%for all $\la, \mu \in \D^d$ if and only if $\ph$ is in the Schur-Agler class.
%\item Let $h$ be a function defined on $\Pi_1^d$. Then there exist an orthongally decomposed Hilbert space $\hilbert = \hilbert_1 + \ldots + \hilbert_d$ and an analytic map $v: \Pi_1^d \to \hilbert$ such that 
%\[
%h(z) - \cc{h(w)} = \sum_{i=1}^d (z_i - \cc{w}_i)\ip{v_i(z)}{v_i(w)}
%\]
%if and only if $h \in \mathcal L_d$.
%\end{enumerate}
%\end{theorem}
%The existence of these models is proved via a lurking isometry argument (see e.g. \cite{ag90, amyloew}).
From models one obtains representations of functions, such as those given in Theorem \ref{oldnevreps} above.

The theory of models was executed in the free case for bounded functions on polynomially convex domains in Agler and {\mc}Carthy \cite{agmc_gh}.
The specific polynomially convex domain of interest used to study certain classes of free functions is the free polydisk
\[
\mathcal B^d = \{X \in \M^d: \norm{X_i} < 1, i = 1, \ldots, d\}.
\]
We obtain representations for free Pick functions by a Cayley transform of these models via
methods developed in \cite{aty13}.




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




We consider matrix monotone functions, which are related to Pick functions by L\"owner's theorem.
A bounded Borel function $f: (a,b) \to \R$ is \emph{matrix monotone} if
$f(X) \leq f(Y)$
 for any pair of matrices
$X, Y \in \M_n(\mathbb{C})$ such that $X \leq Y.$
In \cite{lo34}, Charles L\"owner showed the following theorem.
\begin{theorem}[L\"owner\cite{lo34}]
Let $f: (a,b) \to \R$ be a bounded Borel function. If $f$ is matrix monotone, then $f$ analytically continues to the upper half plane
as a function in the the Pick class.
\end{theorem}
For a modern treatment, see e.g. \cite{don74,bha97,bha07}. L\"owner's theorem has deep connections with science and engineering.
Wigner and von Neumann applied L\"owner's theorem to the quantum theory of collisions \cite{wigner}. Other applications have been seen in the theory of wireless networks \cite{Jorswieck2007f, Boche2004e}.

L\"owner's theorem has been generalized to several commuting functional calculi.
Agler, {\mc}Carthy and Young proved that matrix monotone functions defined on commuting tuples of matrices extend
to functions in the L\"owner class \cite{amyloew}. Others have studied matrix monotonicity on an alternate commutative functional calculus involving tensor products \cite{han03,kor61,siva02}.

We prove a free analogue of L\"owner's theorem in several noncommuting variables.
We consider functions on domains contained in the \emph{real matrix universe,}
	$$\RR^d := \{X \in \M^d |  X_i = X_i^*, i =1 \ldots d\}.$$
A free set $D\subset \RR$ is a \emph{real free domain} if $D \cap \RR^d$ is open in the space $\RR^d_n.$
We prove L\"owner's theorem for real analytic free functions on convex sets.  We note that a real free function 
is analytic if it has a bounded extension to a neighborhood of $D$ in the space $\M^d$ \cite{vvw12}.

We show that L\"owner's theorem holds on convex free sets. Convex free sets have been an object of recent work following the trend in semidefinite programming. For example, Helton and McCullough \cite{heltmc12} showed that semialgebraic convex sets are LMI domains, a generalization of Lasserre's result in the commutative case \cite{las01}. An LMI domain is the set of tuples of self-adjoint  $X_i$ such that
$
\sum A_i \otimes X_i \leq A_0
$
where each $A_i$ is symmetric.

Our generalization of L\"owners theorem is given below.
\begin{theorem}\label{freelow}
Let $D$ be a convex free set of self-adjoint matrices in $\RR^d$.
A real analytic free function $f: D \rightarrow \RR$ is matrix monotone if and only if
$f$ analytically continues to $\Pi^d$ as a function in the the Pick class.
\end{theorem}
This follows from Theorem \ref{lowTheorem} applied to functions on convex domains.
We remark that the representations which correspond to our analogue of Theorem \ref{oldnevreps} can be used to manufacture  concrete formulas for monotone functions similar
to the representations of rational matrix convex functions in work of Helton, McCullough and Vinnikov
\cite{helmcvin06}, which show that rational matrix convex functions are all obtained
by taking the Schur complement of a monic LMI.
In the classical theory, there is a strong connection 
between convex and monotone functions \cite{bha97,kraus36}, which seems to be suggested again here.

For real free analytic functions on convex sets, matrix monotonicity is equivalent to local matrix monotonicity.
Let $Df(X)[H]$ be derivative at a matrix $X$ in the direction $H.$
A free function is \emph{locally matrix monotone} when 
	\[
		Df(X)[H] \geq 0,
	\]
for all $X \in \RR^d$, whenever $H\in \RR^d$ such that each $H_i\geq 0.$

Our proof of Theorem \ref{freelow} constructs a model for locally monotone real analytic free function.
We now sketch the proof in one variable to describe ideas important to the proof.

Given the power series of a monotone function, we construct an explicit model for the function.
Consider an analytic function
\[
f(x) = \sum_{i=0}^\infty a_i x^i
\]
defined on a neighborhood of the closed disk.
We seek to study the formula,
\beq
f'(x) =
\bpm 1 \\ x \\ x^2 \\ \vdots \epm \bbm a_1 & a_2 & a_3 & \ldots \\ a_2 & a_3 & \phantom\ldots & \ldots \\ a_3 & \phantom a &  & \phantom a  \\ \vdots & \vdots & \phantom a & \ddots \ebm \bpm 1 \\ x \\ x^2 \\ \vdots \epm,
\eeq
in the free case. We note the derivative at a matrix $X$ in the direction $H$ is given by the formula,
\beq \label{hampos2}
Df(X)[H] =
\bpm 1 \\ X \\ X^2 \\ \vdots \epm \bbm a_1H & a_2H & a_3H & \ldots \\ a_2H & a_3H & \phantom\ldots & \ldots \\ a_3H & \phantom a &  & \phantom a  \\ \vdots & \vdots & \phantom a &  \ddots \ebm \bpm 1 \\ X \\ X^2 \\ \vdots \epm,
\eeq
and establish that
\beq \label{hampos}
\bbm a_1 & a_2 & a_3 & \ldots \\ a_2 & a_3 & \phantom\ldots & \ldots \\ a_3 & \phantom a &  & \phantom a  \\ \vdots & \vdots & \phantom a &  \ddots \ebm \geq 0.
\eeq
When \eqref{hampos} is satisfied, the formula \eqref{hampos2} for $f'$
implies that $f$ can be analytically continued to the upper half plane as a Pick function via the theory of models \cite{ampi}.
If Equation \eqref{hampos} is satisfied, the expression \eqref{hampos2} is called a \emph{Hamburger model}.
In one variable, \emph{Hamburger model} for a function defined on a neighborhood
of the closed disk is an expression for the derivative of the form
\beq \label{hambonta}
Df(X)[H] =
\bpm 1 \\ X \\ X^2 \\ \vdots \epm \bbm a_{11}H & a_{12}H & a_{13}H & \ldots \\ a_{21}H & a_{22}H & \phantom\ldots & \ldots \\ a_{31}H & \phantom a &  & \phantom a  \\ \vdots & \vdots & \phantom a &  \ddots \ebm \bpm 1 \\ X \\ X^2 \\ \vdots \epm.
\eeq
where $(a_{ij})_{ij}$ is postive semidefinite.
We construct a Hamburger model in Section \ref{construction}, which is unique among expressions of the
form \eqref{hambonta}, irrespective of whether $(a_{ij})_{ij}$ is postive semidefinite or not.
In Section \ref{hankel}, we contruct a candidate for the Hamburger model from the power series for a function, which 
must be equal to the model obtained in Section \ref{construction} by uniqueness.


To construct the Hamburger model, we establish a sum of squares representation
\beq\label{sosDer}
	Df(X)[H] = \sum_{k=0}^{\infty} f_k\ad H f_k,
\eeq
and then reduce it algebraically to the model itself.
This method is modeled on the theory of Positivstellensatz\"e.
In \cite{helmc04}, Helton and McCullough showed the following Positivstellensatz, a generalization of a results of Schm\"udgen \cite{schmu91} and Putinar \cite{put93} to the free case.
\begin{theorem}[Helton, McCullough \cite{helmc04}]
Let $Q$ be a family of free polynomials with the technical assumption that the norm of $X$ such that $q(X)\geq 0$ is bounded.
If $f(X)\geq 0$ whenever all $q\in Q$ satisfy $q(X)\geq 0,$ then
$$f = \sum g^*_ig_i + \sum h^*_jq_jh_j$$
for some finite sequences of free polynomials $g_i,$ $h_j,$ and $q_j$ where each $q_j\in Q.$
\end{theorem}
We emulate the commutative L\"owner theorem \cite{amyloew} by working locally, and
obtain a sum of squares representation as in equation \eqref{sosDer}.

However, we differ in that our method is constructive. Typically, the generation of sum of squares representations or models follows from the Hahn-Banach theorem via a convexity argument. In fact, free versions of the Hahn-Banach theorem exist, such as the Effros-Winkler theorem \cite{effwink}, for which generalizations of the classical argument for the existence of models have been executed \cite{heltmc13}.

Instead, we consider the Choi-Kraus representation theorem \cite{bha07}.
A map $L: \M_n \rightarrow \M_n$ is called \emph{positive} if
	$H\geq 0 \Rightarrow L(H) \geq 0.$
A map $L: \M_n \rightarrow \M_n$ is said to be \emph{completely positive} if the extension of
$L$ to $L^m: \M_n \otimes \M_m \rightarrow \M_n \otimes \M_m$ given on simple tensors by the formula
	$$L^m(A \otimes B) = L(A) \otimes B$$
is positive for every $m.$
\begin{theorem}[Choi\cite{cho72}, Kraus \cite{kraus71}] \label{choi}
A completely positive linear map $L: \M_n \rightarrow \M_n$ can be written in the form
\[
L(H) = \sum V_i\ad H V_i.
\]
\end{theorem}

In one variable, since $Df(X)[H]$ is completely positive in $H,$
along with the homomorphism theory of finite dimensional $C\ad$-algebras\cite{da06},
Theorem \ref{choi} is used to derive the equation \eqref{sosDer} locally, by establishing the $V_i$ are derived from free polynomials $u_i(X).$
So,
\beq\label{sosDer2}
	Df(X)[H] = \sum_k u_k(X)\ad H u_k(X).
\eeq
The theory of establishing equation \eqref{sosDer2} for locally monotone functions corresponds to Lemma \ref{finitehamburger}.

We now introduce the \emph{free coefficient Hardy space} $H^2_d$, the set of free power series in $d$ variables with coefficients in $l^2.$
The free coefficient Hardy space generalizes the classical Hardy space $H^2,$ the set of functions on the disk
whose power series coefficients are in $l^2.$ The classical Hardy space has many important properties, however most important to us
are the Szeg\"o kernels, $k_x \in H^2$ such that $\ip{f}{k_x}= f(x).$
We establish the theory of Szeg\"o kernels for $H^2_d.$ For a given $X \in \M^d_n$ we obtain $k^{ij}_X \in H_d^2$
such that $\ip{f}{k^{ij}_X}= f(X)_{ij}$ for $i,j \leq n,$ the \emph{Szeg\"o kernels at $X$.}
The theory of free coefficient Hardy space codifies previously studied geometry of a vector of monomials, which was
used in the proof that positive free polynomials are sums of squares \cite[Section 2]{heltonPositive} and the proof of the noncommutative Schwarz lemma \cite{hkms09}.
For example, in one variable, define $m_X$ to be the list of monomials written as a column vector. That is,
	$$m_X = \bpm 1 \\ X \\ X^2 \\ \vdots \epm.$$
For any $f\in H^2_1,$ there is a $u\in l^2$ such that $$f(X) = u^*m_X.$$
Via this duality, the theory of $m_X$ is, for our purposes, the theory of the free coefficient Hardy space.
The general theory of the free coefficient Hardy space is given in Section \ref{fchardy}. 

Note that each $u_k(X)$ from formula \eqref{sosDer2} can be written in the form of a tensored inner product,
\beq
u_k(X) = (\flattensor{v_k^*}{I})
\bpm 1 \\ X \\ X^2 \\ \vdots \epm
= \bpm v_{k1}I & v_{k2}I & v_{k3}I & \ldots \epm
\bpm 1 \\ X \\ X^2 \\ \vdots \epm
\eeq
where $v_k \in H_1^2$ is the vector of coefficients the polynomial of $u_k.$
The decomposition allows equation \eqref{sosDer2} to be written in the form of equation \eqref{hampos2},
\beq \label{hambonta2}
Df(X)[H] =
\bpm 1 \\ X \\ X^2 \\ \vdots \epm \bbm a_{11}H & a_{12}H & a_{13}H & \ldots \\ a_{21}H & a_{22}H & \phantom\ldots & \ldots \\ a_{31}H & \phantom a &  & \phantom a  \\ \vdots & \vdots & \phantom a &  \ddots \ebm \bpm 1 \\ X \\ X^2 \\ \vdots \epm,
\eeq
where the matrix $(a_{ij})_{ij}$ is positive semidefinite since $(a_{ij})_{ij} = \sum v_k v_k\ad.$

The matrix $(a_{ij})_{ij}$ in formula \eqref{hambonta2} is unique when restricted the space
spanned by the Szeg\"o kernels at $X.$
As the spectrum of $X$ grows, the Szeg\"o kernels exhaust the space and we obtain one
$(a_{ij})_{ij}$ that satisfies equation \eqref{hambonta} for all $X$ that must agree with equation \eqref{hampos2} by uniqueness.
Since $(a_{ij})_{ij}$ is positive, equation \eqref{hampos} is satisfied.
Since equation \eqref{hampos} is satisfied, the theory of
models allows us to conclude that $f$ extends to the upper half plane as a Pick function.
The full construction is given in Section \ref{construction}.

The paper is structured as follows. In Section \ref{background} we describe free analysis in detail and how it relates to the classical
functional calculus. In Section \ref{foundations}, we develop build the foundations of our paper. The begins with a discussion of
the free coefficient Hardy space with an example in one variable. Then, we establish the \emph{lurking isometry argument,} a tool
to represent functions, via the Hardy space techniques. We then use the lurking isometry to establish a formula
for free Herglotz functions, a class of functions related to free Pick functions, which imply the Nevanlinna representations.
In Section \ref{NevSect}, we prove our Nevanlinna representations, and characterize them using asymptotic behavior.
In Section \ref{LOWNER}, we prove L\"owner's theorem, using the method described above.

















